LIV-GaussMap: LiDAR-Inertial-Visual Fusion for Real-time 3D Radiance Field Map Rendering

We introduce an integrated precise LiDAR, Inertial, and Visual (LIV) multimodal sensor fused mapping system that builds on the differentiable \pre{surface splatting }\now{Gaussians} to improve the mapping fidelity, quality, and structural accuracy. Notably, this is also a novel form of tightly coupled map for LiDAR-visual-inertial sensor fusion. This system leverages the complementary characteristics of LiDAR and visual data to capture the geometric structures of large-scale 3D scenes and restore their visual surface information with high fidelity. The initialization for the scene's surface Gaussians and the sensor's poses of each frame are obtained using a LiDAR-inertial system with the feature of size-adaptive voxels. Then, we optimized and refined the Gaussians using visual-derived photometric gradients to optimize their quality and density. Our method is compatible with various types of LiDAR, including solid-state and mechanical LiDAR, supporting both repetitive and non-repetitive scanning modes. Bolstering structure construction through LiDAR and facilitating real-time generation of photorealistic renderings across diverse LIV datasets. It showcases notable resilience and versatility in generating real-time photorealistic scenes potentially for digital twins and virtual reality, while also holding potential applicability in real-time SLAM and robotics domains. We release our software and hardware and self-collected datasets to benefit the community.

==> sec/gpu.tex <==


\subsubsection{GPU Memory occupation with keyframe selector}

% \begin{table*}[htp!]
% \centering
% \caption{GPU Memory occupation with keyframe selector}
% \begin{tabular}{c c|c c c c c c}
% \hline
% Metric & Method & HKU outdoor & HKU indoor & UST indoor & UST outdoor & UST SS & Avg.\\
% \hline
% {\begin{minipage}{2cm}\centering PSNR\\(Interpolate)\end{minipage}}
% &NA&NA&NA&NA&NA&NA&NA\\
% {\begin{minipage}{2cm}\centering PSIM\\(Interpolate)\end{minipage}}
% &NA&NA&NA&NA&NA&NA&NA\\
% {\begin{minipage}{2cm}\centering LPIPS\\(Interpolate)\end{minipage}}
% &NA&NA&NA&NA&NA&NA&NA\\
% {\begin{minipage}{2cm}\centering PSNR\\(Extrapolate)\end{minipage}}
% &NA&NA&NA&NA&NA&NA&NA\\
% {\begin{minipage}{2cm}\centering PSIM\\(Extrapolate)\end{minipage}}
% &NA&NA&NA&NA&NA&NA&NA\\
% {\begin{minipage}{2cm}\centering LPIPS\\(Extrapolate)\end{minipage}}
% &NA&NA&NA&NA&NA&NA&NA\\
% Memory &NA&NA&NA&NA&NA&NA&NA\\
% \hline
% \end{tabular}
% \label{tab:GPU}
% \end{table*}


% As indicated in Table~\ref{tab:GPU}, the keyframe selection allows for identifying new observation points based on a certain threshold for displacement and angle. This approach effectively reduces GPU memory usage while maintaining a negligible impact on the PSNR.
